SinGAN: Learning a Generative Model from a Single Natural Image

We introduce SinGAN, an unconditional generative model that can be learned from a single natural image. Our model is trained to capture the internal distribution of patches within the image, and is then able to generate high quality, diverse samples that carry the same visual content as the image. SinGAN contains a pyramid of fully convolutional GANs, each responsible for learning the patch distribution at a different scale of the image. This allows generating new samples of arbitrary size and aspect ratio, that have significant variability, yet maintain both the global structure and the fine textures of the training image. In contrast to previous single image GAN schemes, our approach is not limited to texture images, and is not conditional (i.e. it generates samples from noise). User studies confirm that the generated samples are commonly confused to be real images. We illustrate the utility of SinGAN in a wide range of image manipulation tasks.

==> SM.tex <==
\section{Additional Information}

\subsection{Optimization}
At each scale, the weights of the generator and discriminator are initialized to those from the previous trained scale (except for the coarsest scale or when changing the number of kernels, in which cases we use random initialization). We train each scale for 2000 iterations. In each iteration we alternate between 3 gradient steps for the generator and 3 gradient steps for the discriminator. We use the Adam optimizer \cite{kingma2014adam} with a learning rate of $0.0005$ (decreased by a factor of $0.1$ after $1600$ iterations) and momentum parameters $\beta_1=0.5, \beta_2=0.999$. The weight of the reconstruction loss is $\alpha = 10$, and the weight of the gradient penalty in the WGAN loss is $0.1$. Training takes about $30$ minutes on a 1080TI GPU for an image of size $256\times256$ pixels, and the generation at test time is well under one second per image.

\subsection{Boundary conditions and the effect of padding}
The type of padding used within SinGAN's generators highly influences the diversity among generated samples at the corners (the net learns to associate the image structures at the corners with the artificial edges caused by the padding). Figure~\ref{fig:padding} illustrates this effect by depicting the standard deviation among generated samples for each location in the image. %A fully convolutional net fed with spatial random noise cannot associate structures with specific locations in the image (a shift in the input noise will always cause a shift in the output). This is true, however, only away from the boundaries. When using zero padding, we create artificial edges at the borders, which the net \emph{can} learn to associate with the specific structures.
%can be used to enforce boundary conditions and control the amount of variability at the image's borders.
As can be seen, zero padding in each layer leads to very small variability at the corners. This effect is reduced when, instead of padding within the layers, we zero-pad the inputs to the generator (both image and noise) by half the net's receptive field from each side. This is our default setting for generating samples. Finally, if the input image is zero-padded this way while the input noise is padded by noise (\ie taken to be larger), then the effect is further reduced. %, but may sometimes cause artifacts at the boundaries.
We use this configuration for generating animations.

%This helps the generator identify the image borders, and thus serves as a fixed boundary condition for the generation process. Figure~\ref{fig:padding} shows the effect of this padding scheme. Using zero padding at each convolution layer decreases the variability of the generated image. Padding with noise (\ie producing $z^n$ of larger size) insert artifacts to the image. Initially zero padding the input instead (our final setting) helps to generate high quality images with nice structure variability. 

\begin{figure}[h!]
    \center
	\includegraphics[width=0.8\textwidth]{padding.pdf}
	\caption{\textbf{Effect of padding.} The padding configuration highly effects the diversity between samples at the corners. Zero padding in each convolutional layer (layer padding) leads to only minor variability at the corners. Padding only the input to the net (initial padding), leads to somewhat increased variability at the corners. Finally, padding by noise, leads to high variability.}
	\label{fig:padding}
\end{figure}

\begin{figure}[h!]
    \center
	\includegraphics[width=0.8\textwidth]{manipulation_scheme.pdf}
	\caption{\textbf{Image manipulation using SinGAN.} Once a SinGAN model is trained, we can inject an image to one of its coarser scales so as to match its patch distribution to that of the training image. In this example, we feed a downsampled version of a horse image (bottom left) into the $7$th scale of a $10$-scale SinGAN model that was trained on a Zebra image (bottom right). As the this input propagates through the generation pyramid, stripes are gradually added to the horse, which grant it the appearance of a Zebra.}
	\label{fig:manipulation_scheme}
\end{figure}

\subsection{Effect of the injection scale for image manipulation}
In all image manipulation tasks illustrated in the paper, we inject (a possibly downsampled version of) an image into the generation pyramid at some scale $n<N$, and feed forward %this input image in the following levels, 
it through the generators up to the finest scale. This paradigm is illustrated in Fig.~\ref{fig:manipulation_scheme}, where a SinGAN trained on a single Zebra image, adds stripes to a horse injected at a coarse scale. %, so as to match its patch distribution to that of the training image. 
Different injection scales lead to different effects. We demonstrate this in Fig.~\ref{fig:manipulation_scale} in the context of harmonization, paint-to-image, and image editing. As can be seen, the coarser the injection scale, the larger the structures that SinGAN can modify so as to match the statistics of patches in the generated to the training image. Injection at fine scales, only modifies small scale structures and textures, while leaving the global structure intact.

\begin{figure}
	\includegraphics[width=1\textwidth]{manipulation_scale.pdf}
	\caption{\textbf{Effect of the injection scale for image manipulation.} In applications such as harmonization (top), paint-to-image (middle), and editing (bottom), the coarser the scale we inject the input image, the larger the structures that get modified. When the input is injected at fine scales, only the fine textures get modified while the global structure remains fixed.}
	\label{fig:manipulation_scale}
	\vspace{10cm}
\end{figure}

\subsection{Animation from a single image}
To animate a single image $x$, we introduce smooth random changes to SinGAN's noise maps, while restricting them to remain close to the noise maps that generate $x$. Those perturbations produce images with similar layout, and thus create a sequence of images with gradually changed composition. Specifically, denoting by $z_n(t)$ the $n$th scale noise map at time $t$, we construct our random walk as
%\begin{eqnarray*}
%[z_n]_i= \left\{ 
%\begin{matrix}
%{z_n^{rec}} \quad &i=0\\ 
%\alpha z_n^{rec} + (1-\alpha)([z_n]_{i-1}+[z_n]_i^{\text{diff}})  \quad &i\geq 1 \\
%\end{matrix} \right 
%\\ 
%[z_n]_i^{\text{diff}} = \beta ([z_n]_{i-1}-[z_n]_{i-2})+ (1-\beta) z_n^{\text{rand}} 
%\end{eqnarray*}
\begin{align*}
z_n(t+1)&= \alpha z_n^{rec} + (1-\alpha)\left(z_n(t)+z_n^{\text{diff}}(t+1)\right), \nonumber\\
z_n^{\text{diff}}(t+1) &= \beta \left(z_n(t)-z_n(t-1)\right)+ (1-\beta) u_n(t) 
\end{align*}
where $z_n(0)=z_n^\text{rec}$ and $u_n(t)$ is a an iid sequence of noise maps having the same dimensions as $z_n(t)$. Here, $\alpha$ determines how close the frames of the sequence remain to $x$, whereas $\beta$ controls the smoothness and rate of change in the generated clip. Note that similarly to the other image manipulation tasks, here as well we can start the animation from different scales so as to obtain different effects. Please see the supplementary video for animation results.

%Pay attention that in this application the generation can be started at different scales $n$. This, as well as changing the parameters $\alpha, \beta$ can control the variability between frames. Please see the attached pptx file for results.




\newpage
%\section{\Large{Additional Results}}
\section{Additional Results}
%We next provide additional experimental results. 
%\newpage
\subsection{Random Samples}
%\newpage

\begin{figure}[h!]
\center
	\includegraphics[width=1\textwidth]{samples1.pdf}
	%\caption{\textbf{Super-resolution.}}
	%\label{fig:SR}
\end{figure}
\vspace{3cm}
\begin{figure}[h!]
\center
	\includegraphics[width=1\textwidth]{samples2.pdf}
	%\caption{\textbf{Super-resolution.}}
	%\label{fig:SR}
\end{figure}
\vspace{3cm}
\begin{figure}[h!]
    \center
	\includegraphics[width=0.8\textwidth]{HR1.pdf}
	%\label{fig:harmonization}
\end{figure}
\begin{figure}[h!]
    \center
	\includegraphics[width=0.75\textwidth]{HR2.pdf}
	%\label{fig:harmonization}
\end{figure}
%\begin{figure*}[h!]
%    \center
%	\includegraphics[width=0.82\textwidth]{HR3.pdf}
	%\label{fig:harmonization}
%\end{figure*}
\begin{figure}[h!]
    \center
	\includegraphics[width=0.8\textwidth]{HR4.pdf}
	%\label{fig:harmonization}
\end{figure}



\newpage
\subsection{Samples at arbitrary dimensions}
%different effect than the task of image retargeting: (i) our resizing is stochastic (\ie volcano) (ii) for expansions, SinGAN generates new image structures (iii) for reduction, we are not restrict to the original image structure.
%\newpage
Using SinGAN, we can generate samples of arbitrary size and aspect ratio. While this is superficially similar to retargeting, the two tasks are distinct. We illustrate this below through comparison to seam carving \cite{avidan2007seam}. In our case, the samples are \emph{random} and are not optimized to maintain salient objects or strong edges. This often leads to plausible configurations that do not appear in the input image. In image retargeting, on the other hand, structures are typically restricted to those appearing in the image, and may deform unrealistically at extreme aspect ratios.


\begin{figure}[h!]
\center
	\includegraphics[width=1\textwidth]{SC3_1.pdf}
	%\caption{\textbf{Generation vs.~retargeting.} Using SinGAN, we can generate samples of arbitrary size and aspect ratio. While superficially similar to retargeting, the two tasks are distinct, as we illustrate here through comparison to seam carving \cite{avidan2007seam}. In our case, the samples are \emph{random} and are not optimized to maintain salient objects or strong edges. This often leads to plausible configurations that do not appear in the input image. In image retargeting, on the other hand, the structures are typically restricted to those appearing in the image.}
	%\label{fig:SR}
\end{figure}
%\vspace{3cm}
\begin{figure}[h!]
\center
	\includegraphics[width=1\textwidth]{SC3_2.pdf}
	%\caption{\textbf{Generation vs.~retargeting.}}
	%\label{fig:SR}
	\vspace{3cm}
\end{figure}


%\newpage
%\subsection{High Resolution Samples}
%\newpage

\subsection{AMT Survey Images}
%\newpage\
%\vspace{-2.5cm}

\begin{figure}[h!]
\center
%\vspace{-2.5cm}
	\includegraphics[width=1\textwidth]{AMT1.pdf}
	%\caption{\textbf{Super-resolution.}}
	%\label{fig:SR}
	\vspace{1.cm}
\end{figure}
%\vspace{3cm}

\begin{figure}[h!]
\center
	\includegraphics[width=1\textwidth]{AMT2.pdf}
	%\caption{\textbf{Super-resolution.}}
	%\label{fig:SR}
	\vspace{1.4cm}
\end{figure}

\begin{figure}[h!]
\center
	\includegraphics[width=1\textwidth]{AMT3.pdf}
	%\caption{\textbf{Super-resolution.}}
	%\label{fig:SR}
	\vspace{1.4cm}
\end{figure}
%\vspace{3cm}


\subsection{Super-resolution \vspace{0.1cm}}
%\newpage
%\vspace{3cm}

\begin{figure}[h!]
%\vspace{0.2cm}
\center
	\includegraphics[width=0.95\textwidth]{SR1.pdf}
	%\caption{\textbf{Super-resolution.}}
	%\label{fig:SR}
	\vspace{0.19cm}
\end{figure}
%\vspace{3cm}

\begin{figure}[h!]
\center
	\includegraphics[width=1\textwidth]{SR2_2.pdf}
	%\caption{\textbf{Super-resolution.}}
	%\label{fig:SR}
	%\vspace{3cm}
\end{figure}
%\vspace{3cm}

%\newpage
\subsection{Harmonization}
%\newpage 

\begin{figure*}[h!]
\center
	\includegraphics[width=1\textwidth]{harmonization_SM.pdf}
	\label{fig:harmonization1}
    %\vspace{3cm}
\end{figure*}


\begin{figure*}[h!]
\center
	\includegraphics[width=1\textwidth]{harmonization_SM2.pdf}
	\label{fig:harmonization2}
    %\vspace{3cm}
\end{figure*}

%\vspace{5cm}

%\begin{figure*}[h!]
%\center
%	\includegraphics[width=1\textwidth]{Figures/harmonization_3.pdf}
%	\label{fig:harmonization}
%\end{figure*}
%\vspace{6cm}
%\begin{figure*}[h!]
%\center
%	\includegraphics[width=1\textwidth]{Figures/harmonization_4.pdf}
%	\label{fig:harmonization}
%\end{figure*}
%\vspace{3cm}


%\newpage
\subsection{Editing}
%\newpage
\begin{figure*}[h!]
\center
	\includegraphics[width=0.87\textwidth]{editing1.pdf}
	%\label{fig:harmonization}
	%\vspace{3cm}
\end{figure*}

%\vspace{3cm}

\newpage
%\begin{figure*}[h!]
%\center
%	\includegraphics[width=0.9\textwidth]{Figures/editing2.pdf}
%	\label{fig:harmonization}
%\end{figure*}
%\vspace{3cm}

%\newpage
\subsection{Paint to Image}
%\newpage
\begin{figure*}[h!]
\center
	\includegraphics[width=0.65\textwidth]{paint_SM.pdf}
	\label{fig:paint}
	%\vspace{3cm}
\end{figure*}

%\vspace{3cm}

%\newpage
\subsection{Experimental Settings}
The tables below report the settings used for each of the results presented in the main text as well as in this supplementary material. For each application, we specify the scale in which the input image was injected and the total number of scales we used for SinGAN's generation pyramid.

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Image & Injection scale & Total number of scales  \\
    \hline
    Tree (also Fig.~2, main text)& $n = 1$ & $N =9$\\
    Two Dolphins (also Fig.~13, main text)& $n = 3$ & $N = 9$\\
    Single Dolphin & $n = 3$ & $N = 9$\\
    Fox & $n = 2$ & $N = 8$\\
    Airplane & $n = 2$ & $N = 8$\\
    Butterfly & $n = 2$ & $N = 8$\\
    Eagle & $n = 2$ & $N = 8$\\
    Spaceship (also Fig.~13, main text)& $n = 3$ & $N = 8$\\
    Hat & $n = 4$ & $N = 9$\\
    Lemon & $n = 3$ & $N = 7$\\
    Cat & $n = 2$ & $N = 8$\\
    \hline
    \end{tabular}
    \caption{{\bf Harmonization.}}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Image & Injection scale & Total number of scales  \\
    \hline
    Rock1 & $n = 5$ & $N = 7$\\
    Rock2 & $n = 5$ & $N = 7$\\
    Rock3 (also Fig.~12, main text)& $n = 5$ & $N = 7$\\
    Tree & $n = 7$ & $N = 9$\\
    Mountain & $n = 4$ & $N = 8$\\
    Red cliff & $n = 5$ & $N = 9$\\
    Hay & $n = 6$ & $N = 9$\\
    \hline
    \end{tabular}
    \caption{{\bf Editing.}}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Image & Injection scale & Total number of scales  \\
    \hline
    Balloons1 & $n = 7$ & $N=9$\\
    Balloons2 & $n = 5$ & $N=9$\\
    Starry night & $n = 6$ & $N=8$\\
    Rock & $n = 6$ & $N=8$\\
    Tree & $n = 6$ & $N=8$\\
    Birds & $n = 6$ & $N=7$\\
    View (Fig.~2, main text) & $n = 7$ & $N=8$\\
    Pyramids (Fig.~11, main text)  & $n = 6$ & $N=8$\\
    cows (Fig.~11, main text) & $n = 5$ & $N=7$\\
    \hline
    \end{tabular}
    \caption{{\bf Paint to image.}}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Image & Random walk starting scale &  Total number of scales & $\alpha$ & $\beta$  \\
    \hline
    Coral & $n=5$ & $N=7$ & 0.1 &  0.9 \\
    Corals and fish & $n=6$ & $N=8$ & 0.1 &  0.9 \\
    Water  & $n=8$ & $N=8$ & $ 0.1 $ &  $ 0.8 $ \\
    Bush  & $n=6$ & $N=8$ & $ 0.1 $ &  $ 0.9 $ \\
    Trees (slow wind) & $n=6$ & $N=8$ & $0.1 $ &  $0.9 $ \\
    Trees (strong wind) & $n=6$ & $N=8$ & $0.1 $ &  $0.8 $ \\
    Lightning  & $n=7$ & $N=7$ & $ 0.1 $ &  $ 0.9 $ \\
    Fog & $n=5$ & $N=7$ & $ 0.02 $ &  $ 0.95$ \\
    Fire1 & $n=8$ & $N=8$ & $ 0.2 $ &  $ 0.6 $ \\
    %Fire2  & $n=8$ & $N=8$ & $ 0.1 $ &  $ 0.5 $ \\
    Aurora & $n=7$ & $N=8$ & $ 0.1 $ &  $ 0.9 $ \\
    \hline
    \end{tabular}
    \caption{{\bf Single image animation.} See supplementary video.}
\end{table}

%\newpage

==> intro.tex <==

\section{Introduction}

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=1\textwidth]{Figures/manipulation8.pdf}
%	\caption{\textbf{SinGAN for image manipulation.} Other than sampling, SinGAN enables us to manipulate an image for various of tasks such as... using the same generator, which was trained on a single image example.}
%	\label{fig:image_manipulation}
%\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[width=1\textwidth]{Figures/manipulation8.pdf}
	\caption{\textbf{Image manipulation.} SinGAN can be used in various image manipulation tasks, including: transforming a paint (clipart) into a realistic photo, rearranging and editing objects in the image, harmonizing a new object into an image, image super-resolution and creating an animation from a single input. In all these cases, our model observes only the training image (first row) and is trained in the same manner for all applications, with no architectural changes or further tuning (see Sec.~\ref{sec:applications}).}%In all thesAll these executed using the same SinGAN architecture, which was trained on a single image example.}
	\label{fig:image_manipulation} \vspace{-0.35cm}
\end{figure*}

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=1\textwidth]{Figures/manipulation7.pdf}
%	\caption{\textbf{SinGAN for image manipulation.} Other than sampling, SinGAN enables us to manipulate an image for various of tasks such as... using the same generator, which was trained on a single image example.}
%	\label{fig:image_manipulation}
%\end{figure*}

% GANS
Generative Adversarial Nets (GANs) \cite{goodfellow2014generative} have made a dramatic leap in modeling high dimensional distributions of visual data. In particular, unconditional GANs have shown remarkable success in generating realistic, high quality samples when trained on class specific datasets (\eg, faces \cite{liu2015deep}, bedrooms\cite{silberman2012indoor}). However, capturing the distribution of highly diverse datasets with multiple object classes (\eg ImageNet \cite{imagenet_cvpr09}), is still considered a major challenge and often requires conditioning the generation on another input signal \cite{brock2018large} or training the model for a specific task (\eg super-resolution \cite{ledig2017photo}, inpainting \cite{pathak2016context}, retargeting \cite{shocher2018internal}).

%For example, various image manipulation methods have been   \cite{} is often required to make the use of GANs tractable  \cite{dekel2018sparse,perarnau2016invertible,wang2017high,karras2018style}.  %As a consequence, many GAN based image manipulation methods are currently restricted to only one (or a few) object category \cite{}.

% this paper
%To make GAN based methods applicable to arbitrary natural images, here we propose a different route learning from \emph{a single natural image}. % towards making unconditional GAN based methods applicable to a arbitrary natural images. Specifically,
% we explore a different route: Instead of seeking to accommodate ever larger training corpora, %we rather go in the opposite direction. 
Here, we take the use of GANs into a new realm -- \emph{unconditional} generation learned from a \emph{single natural image}. Specifically, we show that the internal statistics of patches within a single natural image typically carry enough information for learning a powerful generative model%that is highly relevant for that image
. \emph{SinGAN}, our new single image generative model, allows us to deal with general natural images that contain complex structures and textures, without the need to %categorize the objects or 
rely on the existence of a database of images from the same class. This is achieved by a pyramid of fully convolutional light-weight GANs, each is responsible for capturing the distribution of patches at a different scale.  Once trained, \emph{SinGAN} can produce diverse high quality image samples (of arbitrary dimensions), which semantically resemble the training image, yet contain new object configurations and structures (Fig.~\ref{fig:teaser}).

%semantically resemble the  %visual content %convey the same visual meaning as of the
%training image (Fig.~\ref{fig:teaser}). %Furthermore, it can be used to perform a wide variety of tasks on the image (Fig.~\ref{fig:image_manipulation}).

%All that is required is a single training image with no prior information. %This thus relieves of the need to collect a new training set every time an image from a new object category is encountered, and is in contrast to conditional GAN models, which are typically trained for a specific task .  

%framework thus relieves of the need to collect a new training set every time an image from a new object category is encountered.

%We explore the use of SinGAN in a variety of applications, and illustrate its ability to cope with highly diverse images can be treated within a as is relieves of the need to collect a new training set every time an image from a new object category is encountered.

%SinGAN contains a pyramid of fully convolutional GANs, each responsible for capturing the distribution of patches at a different scale of the image. This allows generating new samples of arbitrary size and aspect ratio, that have significant variability, while maintaining both the global structure and the fine textures of the training image. 

%In this paper, our goal is different -- we are not aimed at learning the visual distribution of objects across images, as traditional GANs; but rather learning \emph{the internal distribution of patches within a single natural image}. We use the power of adversarial learning and introduce \emph{SinGAN}---a new unconditional GAN model learned from a single input image. From input noise image, our model is designed and trained to generate realistic patch samples, at different scales. Thus, it is able to produce new, high quality image samples, at arbitrary size, which resemble the visual content of the original input image (Figure \ref{fig:teaser}).

Modeling the internal distribution of patches within a single natural image has been long recognized as a powerful prior in many computer vision tasks \cite{zontak2011internal}. Classical examples include denoising \cite{zontak2013separating}, deblurring \cite{michaeli2014blind}, super resolution \cite{glasner2009super}, dehazing \cite{bahat2016blind,freedman2011image}, and image editing \cite{simakov2008summarizing,mechrez2018saliency,he2012statistics,cho2008patch, dekel2015revealing, tlusty2018modifying}. Motivated by these works, here we show how SinGAN can be used within a simple unified framework to solve a variety of image manipulation tasks, including paint-to-image, editing, harmonization, super-resolution, and animation from a single  %\textcolor{green}{training}
image. In all these cases, our model produces high quality results that preserve the internal patch statistics of the training image (see Fig.~\ref{fig:image_manipulation} and our \href{http://webee.technion.ac.il/people/tomermic/SinGAN/SinGAN.htm}{project webpage}). All tasks are achieved with \emph{the same} generative network, that requires no additional information or further training beyond the original training image. 

%\tamar{maybe shorten the following pharagraph, and move the rest to related work section?}
%We note that several single image GAN schemes have been proposed in recent years. However, to the best of our knowledge, no \emph{purely generative} model for \emph{arbitrary natural images} has been suggested to date. In particular, some works proposed conditional single image GANs \cite{} (\ie mapping images to images) for specific tasks, like retargeting \cite{shocher2018internal} or texture expansion \cite{zhou2018non}. Others proposed unconditional GANs (\ie mapping noise vectors to image samples) but only for texture images \cite{bergmann2017learning,jetchev2016texture,li2016precomputed}. As illustrated in Fig.~\ref{fig:texture GAN}, these models do not generate meaningful samples when trained on a general (non-texture) image. SinGAN is thus the first unconditional deep generative model that is applicable for \textcolor{green}{training with a single} natural images.

%The internal distribution of patches in natural images has been long studied and has been shown to be a powerful prior in solving many different computer vision tasks including denoising, deblurring, super resolution X and Y. Motivated by these classical works, we propose a generic generative framework and demonstrate its use in various image manipulation tasks such as harmonization, object rearrangement, paint-to-image. In all these cases, our model produces high quality results that preserve the internal patch statistics of the original input image (see Figure \ref{fig:image_manipulation}). This is achieved with \emph{the same} single generative network, with no additional information or further training.  


%and have been used in many different image manipulation tasks such as image editing \cite{dekel2018sparse,perarnau2016invertible}, semantic manipulation \cite{wang2017high}, image to image translation \cite{isola2017image,wang2017high}, inpainting \cite{}, and style mixing \cite{karras2018style}. In all these cases, the model is

%model

%To obtain good results, this methods are usually exploits...
%Given a single image as input, our SinGAN network is trained on multiple image scales, coarsest to finest, with gradually growing architecture respectively. Thus, it captures rich information from complicated image features, starting from the global image structure to the finest texture. This attribute also enables us to control the generation and manipulation across different image scales.

%Our image specific model allows us to deal with general natural images that contain complex structures and textures, without the need to categorize the objects or rely on the existence of a database of images from the same class. This is a clear advantage over the traditional use of GANs trained on a class specific datasets \cite{arjovsky2017wasserstein,salimans2016improved,gulrajani2017improved,miyato2018spectral}. To generate and manipulate a new image from an unseen category, these methods require a new training set of thousands examples from the desired class. 

%To summarize, %to the best of our knowledge SinGAN is the first unconditional single image generative model.
%our main contributions include: (i) a simple and effective multi-scale framework that allows to capture large image structures as well as \textcolor{green}{delicate} texture\textcolor{green}{s}; (ii) a model that is able to sample realistic realizations of \textcolor{green}{a single} % the 
%training image at arbitrary size; (iii) practical usage in various image manipulation tasks including editing, harmonization, and  super resolution.
%Indeed, current GAN-based image manipulation techniques exemplify their approaches on the same class specific data sets, \eg cityscapes \cite{cordts2016cityscapes}, faces \cite{liu2015deep} and bedrooms \cite{silberman2012indoor}. 

%Tamar
%To summarize,
%our main contributions include: (i) a simple and effective multi-scale framework that allows to capture large image structures as well as \textcolor{green}{delicate} texture\textcolor{green}{s}; (ii) a model that is able to sample realistic realizations \textcolor{green}{ of a single training image example} %of the training image 
%at arbitrary size; 
%(iii) practical usage in various image manipulation tasks including editing, harmonization, and  super resolution.
 


%To allow manipulation of arbitrary images, here we suggest a different route: we claim that a \emph{single image} carries enough information for successfully train a generative model. Thus, generation and various of image manipulation tasks (\eg editing, harmonization, single image animation, super-resolution) can be done by training a simple generative model based on a single image only. This observation is motivated by "classical" image manipulation techniques \cite{efros2001image,hertzmann2001image,darabi2012image,simakov2008summarizing} which models the internal statistics within a single image and do not rely on any external data-set.




%This approach is motivated by the internal statistics based image manipulation techniques \cite{efros2001image,hertzmann2001image,darabi2012image,simakov2008summarizing}. Using our single-image GAN, we could draw samples of images from a single given input images. Exploiting this idea, 

%Using the new approach enables us to generate images which share the same internal statistics with a given single input image (Figure \ref{fig:teaser}), as well as to manipulate an image for various tasks, such as... (Figure \ref{}) while using \emph{the same} single generative network.





==> intro_backups.tex <==
%%%%%%
\section{Introduction}

\begin{figure*}[t]
	\centering
	\includegraphics[width=1\textwidth]{Figures/manipulation8.pdf}
	\caption{\textbf{SinGAN for image manipulation.} Other than sampling, SinGAN enables us to manipulate an image for various of tasks such as... using the same generator, which was trained on a single image example.}
	\label{fig:image_manipulation}
\end{figure*}
% GANS
Generative Adversarial Networks (GANs) \cite{goodfellow2014generative} have made a dramatic leap in modeling high dimensional distributions of visual data. In particular, GAN based models have shown remarkable success in generating realistic, high quality samples when trained on class specific datasets (\eg, faces, bedrooms) and have become an important building block in numerous computer vision tasks \cite{dekel2018sparse,perarnau2016invertible,wang2017high,karras2018style}. However, capturing the distribution of highly diverse datasets with multiple object classes (\eg ImageNet), is still considered to be a major challenge, and often requires class conditioning \cite{} to work well.  %As a consequence, many GAN based image manipulation methods are currently restricted to only one (or a few) object category \cite{}.

% this paper
%To make GAN based methods applicable to arbitrary natural images, here we propose a different route learning from \emph{a single natural image}. % towards making unconditional GAN based methods applicable to a arbitrary natural images. Specifically,
% we explore a different route: Instead of seeking to accommodate ever larger training corpora, we rather go in the opposite direction. 
In this paper, we show that the internal statistics of patches within a \emph{single natural image}, typically carry enough information for learning a powerful generative model that is highly relevant for that image. Specifically, we introduce \emph{SinGAN}---a new unconditional GAN model that is trained on a single image and can then produce diverse high quality samples, which resemble the visual content of that image (Fig.~\ref{fig:teaser}). As we illustrate, once a SinGAN model is trained, it can be used to perform a wide variety of tasks on the image (Fig.~\ref{fig:image_manipulation}). This thus relieves of the need to collect a new training set every time an image from a new object category is encountered, and is in contrast to conditional GAN models, which are typically trained for a specific task (\eg super-resolution, inpainting, retargeting \cite{}).  

%framework thus relieves of the need to collect a new training set every time an image from a new object category is encountered.

%We explore the use of SinGAN in a variety of applications, and illustrate its ability to cope with highly diverse images can be treated within a as is relieves of the need to collect a new training set every time an image from a new object category is encountered.

SinGAN contains a pyramid of fully convolutional GANs, each responsible for capturing the distribution of patches at a different scale of the image. This allows generating new samples of arbitrary size and aspect ratio, that have significant variability, while maintaining both the global structure and the fine textures of the training image. 

%In this paper, our goal is different -- we are not aimed at learning the visual distribution of objects across images, as traditional GANs; but rather learning \emph{the internal distribution of patches within a single natural image}. We use the power of adversarial learning and introduce \emph{SinGAN}---a new unconditional GAN model learned from a single input image. From input noise image, our model is designed and trained to generate realistic patch samples, at different scales. Thus, it is able to produce new, high quality image samples, at arbitrary size, which resemble the visual content of the original input image (Figure \ref{fig:teaser}).

Modeling the internal distribution of patches within a single natural image has been long recognized as a powerful prior in many computer vision tasks. Classical examples include denoising, deblurring, super resolution, dehazing, and image editing. Motivated by these works, here we show how SinGAN can be used within a simple unified framework to solve a variety of image manipulation tasks, including paint-to-image, object rearrangement, harmonization, super-resolution, and animation from a single image. In all these cases, our model produces high quality results that preserve the internal patch statistics of the training image (see Fig.~\ref{fig:image_manipulation}). All tasks are achieved with \emph{the same} generative network, that requires no additional information or further training beyond the original training image. 

We note that several single image GAN schemes have been proposed in recent years. However, to the best of our knowledge, no \emph{purely generative} model for \emph{arbitrary natural images} has been suggested to date. In particular, some works proposed conditional single image GANs \cite{} (\ie mapping images to images) for specific tasks, like retargeting \cite{} or texture expansion \cite{}. Others proposed unconditional GANs (\ie mapping noise vectors to image samples) but only for texture images \cite{}. As illustrated in Fig.~\ref{fig:texture GAN}, these models do not generate meaningful samples when trained on a general (non-texture) image. SinGAN is thus the first unconditional deep generative model that is applicable for natural images.



%The internal distribution of patches in natural images has been long studied and has been shown to be a powerful prior in solving many different computer vision tasks including denoising, deblurring, super resolution X and Y. Motivated by these classical works, we propose a generic generative framework and demonstrate its use in various image manipulation tasks such as harmonization, object rearrangement, paint-to-image. In all these cases, our model produces high quality results that preserve the internal patch statistics of the original input image (see Figure \ref{fig:image_manipulation}). This is achieved with \emph{the same} single generative network, with no additional information or further training.  




%and have been used in many different image manipulation tasks such as image editing \cite{dekel2018sparse,perarnau2016invertible}, semantic manipulation \cite{wang2017high}, image to image translation \cite{isola2017image,wang2017high}, inpainting \cite{}, and style mixing \cite{karras2018style}. In all these cases, the model is

%model

%To obtain good results, this methods are usually exploits...
%Given a single image as input, our SinGAN network is trained on multiple image scales, coarsest to finest, with gradually growing architecture respectively. Thus, it captures rich information from complicated image features, starting from the global image structure to the finest texture. This attribute also enables us to control the generation and manipulation across different image scales.

%Our image specific model allows us to deal with general natural images that contain complex structures and textures, without the need to categorize the objects or rely on the existence of a database of images from the same class. This is a clear advantage over the traditional use of GANs trained on a class specific datasets \cite{arjovsky2017wasserstein,salimans2016improved,gulrajani2017improved,miyato2018spectral}. To generate and manipulate a new image from an unseen category, these methods require a new training set of thousands examples from the desired class. 

To summarize, %to the best of our knowledge SinGAN is the first unconditional single image generative model.
our main contributions include: (i) a simple and effective multi-scale framework that allows to capture large image structures as well as \textcolor{green}{delicate} texture\textcolor{green}{s}; (ii) a model that is able to sample realistic realizations of \textcolor{green}{a single} % the 
training image at arbitrary size; (iii) practical usage in various image manipulation tasks including editing, harmonization, and  super resolution.
%Indeed, current GAN-based image manipulation techniques exemplify their approaches on the same class specific data sets, \eg cityscapes \cite{cordts2016cityscapes}, faces \cite{liu2015deep} and bedrooms \cite{silberman2012indoor}. 

%Tamar
To summarize,
our main contributions include: (i) a simple and effective multi-scale framework that allows to capture large image structures as well as \textcolor{green}{delicate} texture\textcolor{green}{s}; (ii) a model that is able to sample realistic realizations \textcolor{green}{ of a single training image example} %of the training image 
at arbitrary size; 
(iii) practical usage in various image manipulation tasks including editing, harmonization, and  super resolution.
 


%To allow manipulation of arbitrary images, here we suggest a different route: we claim that a \emph{single image} carries enough information for successfully train a generative model. Thus, generation and various of image manipulation tasks (\eg editing, harmonization, single image animation, super-resolution) can be done by training a simple generative model based on a single image only. This observation is motivated by "classical" image manipulation techniques \cite{efros2001image,hertzmann2001image,darabi2012image,simakov2008summarizing} which models the internal statistics within a single image and do not rely on any external data-set.




%This approach is motivated by the internal statistics based image manipulation techniques \cite{efros2001image,hertzmann2001image,darabi2012image,simakov2008summarizing}. Using our single-image GAN, we could draw samples of images from a single given input images. Exploiting this idea, 

%Using the new approach enables us to generate images which share the same internal statistics with a given single input image (Figure \ref{fig:teaser}), as well as to manipulate an image for various tasks, such as... (Figure \ref{}) while using \emph{the same} single generative network.






%%%%%%%
\section{Introduction}

\begin{figure*}[t]
	\centering
	\includegraphics[width=1\textwidth]{Figures/manipulation2.pdf}
	\caption{\textbf{SinGAN for image manipulation.} Other than sampling, SinGAN enables us to manipulate an image for various of tasks such as... using the same generator, which was trained on a single image example.}
	\label{fig:image_manipulation}
\end{figure*}


In recent years, the task of training generative models for natural images gain much attention, with the introduction of Generative Adverserial Networks (GANs) \cite{goodfellow2014generative} . Correspondingly, GANs become attractive for many image manipulation tasks such as image editing \cite{dekel2018sparse,perarnau2016invertible}, semantic manipulation \cite{wang2017high}, image to image translation \cite{isola2017image,wang2017high}, inpainting \cite{}, style mixing \cite{karras2018style} and more.
%To obtain good results, this methods are usually exploits...
However, while GAN and its variants \cite{arjovsky2017wasserstein,salimans2016improved,gulrajani2017improved,miyato2018spectral} showed promising results, their success is often limited to intra-class image generation. Indeed, when trained on a large and complex dataset (\eg ImageNet \cite{imagenet_cvpr09}) the visual quality of the sampled images is usually unsatisfactory. This limits current GAN based image generation and manipulation approaches to apply only for a class-specific images. In order to manipulate a new image, from a category never seen before, one should collect a new training set containing thousands of examples from the desire class, and spent time and resources on training a new generative model. Indeed, current GAN-based image manipulation techniques exemplify their approaches on the same class specific data sets, \eg cityscapes \cite{cordts2016cityscapes}, faces \cite{liu2015deep} and bedrooms \cite{silberman2012indoor}. 

To allow manipulation of arbitrary images, here we suggest a different route: we claim that a \emph{single image} carries enough information for successfully train a generative model. Thus, generation and various of image manipulation tasks (\eg editing, harmonization, single image animation, super-resolution) can be done by training a simple generative model based on a single image only. This observation is motivated by "classical" image manipulation techniques \cite{efros2001image,hertzmann2001image,darabi2012image,simakov2008summarizing} which models the internal statistics within a single image and do not rely on any external data-set.

Based on this, we suggest a new approach for training GAN given a single natural image, which we coin \emph{SinGAN}. Our model learns to generate images which share the same internal patch-distribution as a given single input image, across multiple scales, and is therefore capable with producing sample images which have the same visual content (Figure \ref{fig:teaser}). Furthermore, the new framework enables to manipulate an image for various tasks (Figure \ref{fig:image_manipulation}) while maintaining the same internal statistics as of the original input image, and by using \emph{the same} single generative network, trained with a single example. 

Given a single image as input, our SinGAN network is trained on multiple image scales, coarsest to finest, with gradually growing architecture respectively. Thus, it captures rich information from complicated image features, starting from the global image structure to the finest texture. This attribute also enables us to control the generation and manipulation across different image scales.

%This approach is motivated by the internal statistics based image manipulation techniques \cite{efros2001image,hertzmann2001image,darabi2012image,simakov2008summarizing}. Using our single-image GAN, we could draw samples of images from a single given input images. Exploiting this idea, 

%Using the new approach enables us to generate images which share the same internal statistics with a given single input image (Figure \ref{fig:teaser}), as well as to manipulate an image for various tasks, such as... (Figure \ref{}) while using \emph{the same} single generative network.




==> method_backup.tex <==
\section{Method}

Our goal is to learn a generative model that captures the internal statistics of a \emph{single} training image $x$. This task is conceptually similar to the conventional GAN setting, except that here the training samples are patches (of $x$) rather than whole images. %aims to generate fake images from a given \emphe{single} input image $y$. As we have only \emphe{one} real image example, we could not train the GAN to sample from an image collection, as done in standard GANs training. Instead, we treat the patches of the real image as our training examples, and wish to generate fake images $x$ with matching image patch distribution across multiple scales. 
Single image GANs have been explored for modeling textures \cite{} via use of Markovian discriminators (patch-GAN) \cite{li2016precomputed,isola2017image}. Here, however, we would like to go beyond textures, and treat general natural images. This requires capturing the statistics of structures at many different scales. To do so, we use a hierarchy of patch-GANs, where each is responsible for capturing the patch distribution at a different scale of $x$. This is illustrated in Fig.~\ref{fig:architecture}. Similar architectures have been used in conventional GAN settings (\eg \cite{karras2017progressive,wang2017high,karras2018style,wang2017high,denton2015deep,huang2017stacked}), but not for single images.

\subsection{Multi-scale architecture}
%Our architecture is similar to that proposed in several recent works \cite{karras2017progressive,wang2017high,karras2018style,wang2017high,denton2015deep,huang2017stacked}, with the distinction that here we use a \emph{single image} GAN for each scale. Specifically, 
%This allows us an accurate generation, as well as the ability to control manipulation across different image scales.
Let $x_1,x_2,\ldots,x_N$ be a pyramid of increasingly coarser versions of $x$, obtained by downsampling $x$ at factors $r,r^2,\ldots,r^N$, respectively, where $r>1$ is some small scaling factor (\eg $4/3$). For convenience, we denote $x_0=x$. For each scale $n$, we have a generator $G_n$ and a corresponding discriminator $D_n$, whose joint goal is to capture the patch statistics of the image $x_n$ at that scale. 

%Here $r>1$ is some scaling factor $r$. We built a pyramid of images \{$y_n$\} composed of downsampled versions of the real image $y$, each serve as the real image example at each scale $n$ correspondingly. We use a Markovian discriminator (patch-GAN) \cite{li2016precomputed,isola2017image} which produces a discrimination \emph{map}, ranking each of the image patch's (with the size of the network's receptive-field) as real or fake. This way, at each of the scales the generator $G_n$ aims to produce a fake image $x_n$ with has the same patch distribution as the input image.   
%At each scale, the generator $G_n$ is trained to generate a fake image $x_n$ by matching the internal images patch statistics of the real image at the current scale $n$. This makes the generator produce images which have the same patch distribution as the give input image across $y$ multiple scales, and   
%Each generator responsible for a specific level of an image pyramid. 

%We will next describe the multi-scale architecture and the training procedure in details.
%The real image example at scale is a downsampled version of the input image, and the input to the generator at each scale is a spatial noise (with the size of the real example), and an upsample version of sample from the previous scale (except for the coarsest core where the input is only spatial noise). 




%\paragraph{Multi-scale training}
%We start with training the coarsest scale $n=0$ and gradually add the next GAN. While training the $n$-th scale, all the previous (already trained) networks remain fixed. 
The GAN at the coarsest scale ($n=N$) is purely generative. Its goal is to capture the global structure and object arrangement in the image (\eg sky at the top, ground at the bottom), by learning the patch distribution within $x_N$. Specifically, its generator $G_N$ maps spatial white Gaussian noise $z_N$ to an image sample $\tilde{x}_N$, 
\begin{align}
\label{eq:GenChain}
\tilde{x}_N= G_N(z_N).
\end{align}
This is done so as to fool its discriminator $D_N$, which attempts to distinguish between generated samples and the real image $x_N$ based on their patch statistics. %Both $z_N$ and $\tilde{x}_N$ have the same dimensions as $x_N$. 

The GANs at all the finer scales ($n<N$) are conditional. The purpose of each of these GANs is to add fine details that do not appear in samples generated at the previous scale. Thus, in addition to spatial noise $z_n$, the generator $G_n$ accepts an upsampled version of the image from the coarser scale, $(\tilde{x}_{n+1})\uparrow^r$. That is, for every $n<N$, the generated sample $\tilde{x}_n$ is obtained as 
\begin{align}
\tilde{x}_{n} = G_n\left(z_n,\,(\tilde{x}_{n+1})\uparrow^r\right).
\end{align}
The discriminator $D_n$, again, attempts to distinguish $\tilde{x}_n$ from $x_n$ based on their patch statistics. 

All the generators have a similar architecture, as depicted in Fig.~\ref{fig:single_scale}. Specifically, the noise $z_n$ is added to the image $(\tilde{x}_{n+1})\uparrow^r$, prior to being fed into a sequence of convolutional layers. This ensures that the GAN does not disregard the noise, as happens when using concatenation \cite{zhu2017unpaired,mathieu2015deep,zhu2017toward}. The role of the convonlutional layers is to generate the details that are missing in~$(\tilde{x}_{n+1})\uparrow^r$ (residual learning). Namely, $G_n$ performs the operation
\begin{equation}\label{eq:}
    \tilde{x}_{n} = (\tilde{x}_{n+1})\uparrow^r  + \,\, \psi_n\left(z_n + (\tilde{x}_{n+1})\uparrow^r\right),
\end{equation}
where $\psi_n$ is a fully convolutional net. Since we only have a single image to train on, we take $\psi_n$ to be light, with 5 conv-blocks of the form Conv($3\times 3$)-BatchNorm-LeakyReLU \cite{ioffe2015batch}. We start with $32$ kernels per block at the coarsest scale $n=N$, and increase this number by a factor of $2$ every $4$ scales. 

%In addition, each generator $G_n, n>0$  learns the residual to the upsampled version of the previous scale $(x_{n-1})\uparrow^r$. Therefore, at each scale the generator is responsible for adding image details on top of the generated image from the previous scale. The effect of the multi-scale scheme is demonstrated in Fig. \ref{fig:multi_scale}. When using a single scale, we only manage to produce the fine texture in the image. As the number of scales increases, the generator manage to capture the image global characteristics.

At test time, the generation of an image sample at the finest scale, involves drawing random noise maps $z_N,z_{N-1},\ldots,z_0$ at all scales. Namely, the generation begins from the coarsest scale $n=N$ and propagates through all the generators until reaching the finest scale. Since the generators are fully convolutional, the generation process is not limited to a specific image size. By changing the size of the noise maps, we can control the output size. This gives us the flexibility to generate images of arbitrary sizes and aspect ratios\footnote{Note that this is not similar to retargeting the image $x$. The samples are random, and are optimized to maintain the patch statistics, not necessarily salient objects in $x$. See SM for comparisons to retargeting methods.}.

 

%we did not train the network to produce optimal retargeted images by any mean. In addition, the generation is stochastic, \ie given a desire output says, we will get random output images. For the comparison, we compare the results for retargeting algorithms in the supplementary material.

%as shown in Fig. \ref{fig:samples}

%Therefore, training can be done on high resolution images, like presented in Fig. \ref{fig:high-res}.

\subsection{Training}
To train our multi-scale architecture, we start from the coarsest scale and proceed sequentially until reaching the finest scale. Once each GAN has finished training, its generator is kept fixed (and the discriminator is discarded). Thus, although the generation at the $n$th scale is affected by all the generators up to this scale, only the parameters of $G_n$ and $D_n$ are updated when training this scale. 

To update the generator $G_n$, we minimize a loss function comprising an adversarial term and a reconstruction term,
\begin{equation}
\label{eq:total Loss}
%\hat{G}_n = 
\min_{G_n}\,\, \mathcal{L}_{\text{adv}}+\alpha\mathcal{L}_{\text{rec}}.
\end{equation}
The adversarial loss $\mathcal{L}_{\text{adv}}$ penalizes for the Wasserstein distance between the distribution of patches in $x_n$ and the distribution of patches in generated samples $\tilde{x}_n$. Specifically, we use the WGAN-GP loss \cite{gulrajani2017improved}, which we found to increase training stability. The reconstruction loss $\mathcal{L}_{\text{rec}}$ insures that there exist some specific set of noise maps, which can produce the image $x_n$.

\paragraph{Adversarial loss}
We use a Markovian discriminator $D_n$ which classifies each of the overlapping patches of its input image as real or fake. The discriminator $D_n$ has the same architecture as the net $\psi_n$ within $G_n$. The patch size is determined by the network's receptive field, which is $11\times11$ in our case. The final discrimination score is calculated by taking the average over the patch discrimination map. Thus the adversarial loss $\mathcal{L}_{\text{adv}}$ for the $n$th scale is
\begin{align}
\label{eq:WGAN}
\max_{D_n}\,\, &\mathbb{E}\left[D_n(\tilde{x}_n)\right]-D_n(x_n)\nonumber\\
&+ \lambda\mathbb{E}\left[(\| \nabla_{\bar x} D_n(\bar x_n) \|_2-1)^2\right],
\end{align}
where $\bar x_n=\gamma x_n + (1-\gamma) \tilde{x}_n$ with $\gamma\sim U(0,1)$ \cite{gulrajani2017improved}, and the expectations are over draws of $\tilde{x}_n$ and $\gamma$. Note that as opposed to the common setting, here we have no expectation over $x_n$, as we only have one training example.
%(which are functions of the random noise maps $\{z_N,\ldots,z_n\}$) and draws

\paragraph{Reconstruction loss}
To stabilize the training, and to drive the samples to be of high quality, we ensure that there exists a specific sequences of noise maps, which generates the input image $x$. We specifically choose $\{z_N^{\text{rec}},z_{N-1}^{\text{rec}}\ldots,z_0^{\text{rec}}\}=\{z^*,0,\ldots,0\}$, where $z^*$ is some fixed noise map (drawn once and kept fixed during training). Denote by $\tilde{x}_n^{\text{rec}}$ the generated image at the $n$th scale when using these noise maps. Then our reconstruction loss $\mathcal{L}_{\text{rec}}$ at the $N$th scale is given by
\begin{equation}
\label{eq:rec}
 \|G_N(z^*)- x_N\|^2,
\end{equation}
and at every other scale $n<N$, is
\begin{equation}
\label{eq:rec}
 \|G_n(0, (\tilde{x}_{n+1}^{\text{rec}})\uparrow^r)- x_n\|^2.
\end{equation}
We also use $\tilde{x}_n^{\text{rec}}$ to determine the standard deviation $\sigma_n$ of the noise $z_n$ in each scale. Specifically, we take $\sigma_n$ to be $\tfrac{1}{10}$ of the root mean squared error (RMSE) between $\tilde{x}_n^{\text{rec}}$ and $x_n$. This gives an assessment of the amount of details that need to be added at that scale. %The effect of the reconstruction loss and the additive noise standard deviation are discussed in Fig. \ref{fig:ablation}

\paragraph{Optimization}
At each scale, the weights of the generator and discriminator are initialized to those from the previous trained scale (except for the coarsest scale or when changing the number of kernels, in which cases we use random initialization). We train each scale for 2000 iterations. In each iteration we alternate between 3 gradient steps of the generator and 3 gradient steps of the discriminator. We use Adam \cite{kingma2014adam} with a learning rate of $0.0005$ (decreased by a factor of $0.1$ after $1600$ iterations) and momentum parameters $\beta_1=0.5, \beta_2=0.999$. The reconstruction loss and the gradient penalty weights are $\alpha = 10$, $\lambda = 0.1$, respectively. Training takes about $30$ minutes on a single 1080TI GPU for an image of size $256\times256$ pixels, and the generation at test time is well under one second per image.

%At inference time, we run the generator exactly as during training. Please note that SinGAN is trained on a single input image only, therefore the batch size is always equals $1$.  


%\begin{equation}
%\label{eq:total Loss}
%%\hat{G}_n = 
%\underset{G_n}{\min}\,\underset{D_n}{\max} \, %\mathcal{L}_{adv}(G_n,D_n)+\alpha\mathcal{L}_{rec}(G_n,y_n).
%\end{equation}

%The ``real'' example at each scale, $y_n$, is a single image: a downsampled version of the input image $y$ by a factor of $r \cdot (N-n)$, correspond to the current scale $n$ and the total number of scale $N$. $x_n$ is the a sample fake image generated from $G_n$. 

%The reconstruction loss $\mathcal{L}_{rec}$ insures there exist an input noise $z_n^{rec}$ which generates the real image $y_n$
%\begin{equation}
%\label{eq:rec}
%\mathcal{L}_{rec}(G_n,y_n) = \|G_n(z_n^{rec})- y_n\|^2.
%\end{equation}
%At the first scale, $z_0^{rec}$ is randomly chosen. At all the following scales $z_n^{rec}=0$. The standard deviation $\sigma_n$ of the input noise $z_n$ is estimated from the value of $\mathcal{L}_{rec}$ at the first training iteration. This gives us an assessment of the amount of details need to be added at the current scale. The effect of the reconstruction loss and the additive noise standard deviation are discussed in Fig. \ref{fig:ablation}



%Equation (\ref{eq:GenChain}) also demonstrates how the generation process is sequential: when sampling a new fake example at the $n$-th scale, we start the generation from the coarsest scale $n=0$ and continue through all the following generation scales to get the current generated image. This is done both in training and inference time.


%maps a spatial noise $z_n$ (with the size of the real example $y_n$), added to an upsample version of the generated image from the previous scale $(x_{n-1})\uparrow^r$, as described in Fig. \ref{fig:single_scale}.

%\begin{eqnarray}
%\label{eq:GenChain}
%x_n= \left\{ 
%\begin{matrix}
%G_0(z_0), \quad &n=0\\ 
%G_n(z_n,(x_{n-1})\uparrow^r), \quad &n\geq 1 
%\end{matrix}
%\right.
%\end{eqnarray}



%Equation (\ref{eq:GenChain}) also demonstrates how the generation process is sequential: when sampling a new fake example at the $n$-th scale, we start the generation from the coarsest scale $n=0$ and continue through all the following generation scales to get the current generated image. This is done both in training and inference time. 





%\paragraph{Architecture}
%Since we train SinGAN on a single example, the architecture of the networks is pretty light: At each scale the generator and discriminator have an identical architecture of 5 conv-blocks of the form Convolution-BatchNorm-LeakyReLU \cite{ioffe2015batch} with a fixed number of kernels of size $3 \times 3$ for all blocks. We start with $32$ kernels per block at the coarsest scale, and increase this number by a factor of $2$ every $4$ scales. The weights of the generator and discriminator at each scale are initialized the previous trained scale (except for the case of changing the number of kernels, and the first scale, where the weights are randomly drawn from normal distribution). 






%controlling the variability 



